Synthesis of Parallel Synchronous Software

In typical embedded applications, the precise execution time of the program does not matter, and it is sufficient to meet a real-time deadline. However, modern applications in information security have become much more time-sensitive, due to the risk of timing side-channel leakage. The timing of such programs needs to be data-independent and precise. We describe a parallel synchronous software model, which executes as N parallel threads on a processor with word-length N. Each thread is a single-bit synchronous machine with precise, contention-free timing, while each of the N threads still executes as an independent machine. The resulting software supports fine-grained parallel execution. In contrast to earlier work to obtain precise and repeatable timing in software, our solution does not require modifications to the processor architecture nor specialized instruction scheduling techniques. In addition, all threads run in parallel and without contention, which eliminates the problem of thread scheduling. We use hardware (HDL) semantics to describe a thread as a single-bit synchronous machine. Using logic synthesis and code generation, we derive a parallel synchronous implementation of this design. We illustrate the synchronous parallel programming model with practical examples from cryptography and other applications with precise timing requirements.

==> sections/ciphersTable.tex <==
\begin{table}[t]
% \vspace{-.5cm}
\caption{Evaluated Encryption Ciphers}
%\vspace{-.2cm}
\centering
\small
\setlength\tabcolsep{8pt}
\begin{tabular}{l|cccc}
\multicolumn{1}{c|}{\textbf{cipher}} & \textbf{block size} & \textbf{key size} & \textbf{rounds} & \textbf{type}    \\ \hline
SIMON                       & 128        & 128      & 68     & Feistel \\
PRESENT                     & 64         & 80       & 31     & SPN     \\
LED                         & 64         & 64       & 32     & SPN     \\
Midori                      & 64         & 128      & 16     & SPN     \\
% DES                         & 64         & 64       & 16     & Feistel    
\end{tabular}
\label{tab:ciphers}
\vspace{-.5cm}
\end{table}

==> sections/pspVsNormal.tex <==
\begin{table}[t]
\centering
% \vspace{+0.5cm}
\caption{Comparison of performance of the PSP and normal implementations of some cryptographic ciphers}
\begin{threeparttable}

% \vspace{-.2cm}
\setlength\tabcolsep{10pt}
\begin{tabular}{l|ccc}
% \cline{2-3}
\multicolumn{1}{c|}{}               & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}time\\ (cycles/byte)\end{tabular}} \\ 
% \cline{2-3}
\multicolumn{1}{c|}{\textbf{cipher}}        & \multicolumn{1}{c}{\textbf{PSP}}     & \multicolumn{1}{c|}{\textbf{normal}} & \multicolumn{1}{c}{\textbf{speedup}} \\ \hline
\multicolumn{1}{l|}{SIMON-128/128} & 744.48    & \multicolumn{1}{c|}{1315.63}  & \multicolumn{1}{c}{1.7$\times$}    \\ 
\multicolumn{1}{l|}{PRESENT-80}    & 399.61    & \multicolumn{1}{c|}{1069.06}  & \multicolumn{1}{c}{2.6$\times$}    \\
\multicolumn{1}{l|}{Midori-64}     & 236.90    & \multicolumn{1}{c|}{2233.38}  & \multicolumn{1}{c}{9.4$\times$}    \\  
% \multicolumn{1}{l|}{LED}           & 546.68 (LED-64)                                         & 2243.19 (LED-80)                        \\ 
% \multicolumn{1}{l|}{DES}           & 218.26                                          &                                \\ 
\end{tabular}

    % \begin{tablenotes}
    % \tnote{1}   \footnotesizee
    %   \item [1] Implementation on RL78 16bit microcontroller. \footnote{https://www.cryptrec.go.jp/report/cryptrec-gl-2003-2016en.pdf}
    % \end{tablenotes}
\end{threeparttable}
\label{tab:pspvsnorm}
\vspace{-.5cm}
\end{table}

%%%%% from benchmarks:
% present:
    % 17105 * 8 / 128
    % cortex m3 
    % pre-computed key
    % FELICS paper
    
% simon:
    % 21050 * 8 / 128
    % rl78 16bit microprocessor
    % key is not pre-computed 
    % https://www.cryptrec.go.jp/report/cryptrec-gl-2003-2016en.pdf  (page 51)

% led:
    % 35891 * 8 / 128
    % cortex m3 
    % pre-computed key
    % FELICS paper

% midori:
    % 17867 * 8 / 64
    % rl78 16bit microprocessor
    % key is not pre-computed 
    % https://www.cryptrec.go.jp/report/cryptrec-gl-2003-2016en.pdf  (page 51)


%%%%% our designs:
% simon: 381175 * 8 / 32 / 128
% present: 102301 * 8 / 64 / 32
% led: 139,949 * 8 / 64 / 32
% midori: 60646 * 8 / 64 / 32
% des: 55874 * 8 / 64 / 32
